Optimal Shrinkage of Eigenvalues in the Spiked Covariance Model

We show that in a common high-dimensional covariance model, the choice of loss function has a profound effect on optimal estimation. In an asymptotic framework based on the Spiked Covariance model and use of orthogonally invariant estimators, we show that optimal estimation of the population covariance matrix boils down to design of an optimal shrinker $\eta$ that acts elementwise on the sample eigenvalues. Indeed, to each loss function there corresponds a unique admissible eigenvalue shrinker $\eta^*$ dominating all other shrinkers. The shape of the optimal shrinker is determined by the choice of loss function and, crucially, by inconsistency of both eigenvalues and eigenvectors of the sample covariance matrix. Details of these phenomena and closed form formulas for the optimal eigenvalue shrinkers are worked out for a menagerie of 26 loss functions for covariance estimation found in the literature, including the Stein, Entropy, Divergence, Frechet, Bhattacharya/Matusita, Frobenius Norm, Operator Norm, Nuclear Norm and Condition Number losses.

==> authors.tex <==

\begin{aug}
\author{\fnms{David}
\snm{Donoho}\thanksref{nsf}\ead[label=e1]{donoho@stanford.edu}}
,
\author{\fnms{Matan}
\snm{Gavish}\thanksref{sgf,nsf}\ead[label=e2]{gavish@cs.huji.ac.il}}
\and
\author{\fnms{Iain}
\snm{Johnstone}\thanksref{nsf}\ead[label=e3]{imj@stanford.edu}}

\thankstext{nsf}{Partially supported by NSF DMS 0906812 (ARRA) and 1407813}
\thankstext{sgf}{Partially supported by a William R. and Sara Hart Kimball
Stanford Graduate Fellowship}
\runauthor{D. Donoho, M. Gavish and I. Johnstone}

\affiliation{Stanford University and Hebrew University}

\address{
D. Donoho and I. Johnstone\\
  Department of Statistics\\
Sequoia Hall\\
390 Serra Mall\\ 
Stanford University\\
Stanford, CA 94305-4065\\
USA\\
\printead{e1}\\
\printead{e3}\\
%\phantom{E-mail:\ }\printead*{e1,e3}
}

\address{
  M. Gavish\\
School of Computer Science and Engineering\\
Hebrew University of Jerusalem\\
Edmond J. Safra Campus\\
Jerusalem 91904\\ 
Israel\\
\printead{e2}\\
%\phantom{E-mail:\ }\printead*{e2}
}



\end{aug}




==> keywords.tex <==
\begin{keyword}[class=AMS]
\kwd[Primary ]{62C20}
\kwd{62H25}
\kwd[; secondary ]{90C25}
\kwd{90C22}
\end{keyword}

\begin{keyword}
  \kwd{Covariance Estimation}
  \kwd{Optimal Shrinkage}
  \kwd{Stein Loss}
  \kwd{Entropy Loss}
  \kwd{Divergence Loss}
  \kwd{Fr\'{e}chet Distance}
  \kwd{Bhattacharya/Matusita Affinity}
  \kwd{Condition Number Loss}
  \kwd{High-Dimensional Asymptotics}
  \kwd{Spiked Covariance}
\end{keyword}



==> loadcounters.tex <==
% this needs \usepackage{xr,refcount} in sourcing doc's preamble

% counter names need to match counters stored in storecounters.tex

% set this to match counters in main file
\newcommand*{\getcounter}[2]{%
  \setcounterref{#1}{#2}% Retrieve label value and store it in a counter
}

\getcounter{thm}{extthm}
\getcounter{cor}{extcor}
\getcounter{defn}{extdefn}
\getcounter{lemma}{extlemma}
\getcounter{prop}{extprop}
\getcounter{figure}{extfigure}





==> packages.tex <==
\RequirePackage[OT1]{fontenc}
\RequirePackage{amsthm,amsmath}
\RequirePackage[numbers]{natbib}
%\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

% my packages
\usepackage{amsmath,amssymb,graphicx,amsthm,ifthen,epstopdf,fancyhdr,color}
\usepackage{epsfig}
\usepackage{etoolbox}
\usepackage{xr,refcount}
\usepackage{amssymb,amsfonts,amsmath,amsthm,amscd,dsfont,mathrsfs}
\usepackage{graphicx,float,psfrag,epsfig,color}
\usepackage{latexsym}
\usepackage{multirow}
\usepackage{palatino}
\usepackage{epstopdf}
\usepackage[bookmarks=true]{hyperref}


%\usepackage[bookmarks=true]{hyperref}
%\usepackage{cite}



